Activity Recognition on Avatar-Anonymized Datasets with Masked Differential Privacy

Privacy-preserving computer vision is an important emerging problem in machine learning and artificial intelligence. Prevalent methods tackling this problem use differential privacy (DP) or obfuscation techniques to protect the privacy of individuals. In both cases, the utility of the trained model is sacrificed heavily in this process. In this work, we present an anonymization pipeline that replaces sensitive human subjects in video datasets with synthetic avatars within context, employing a combined rendering and stable diffusion-based strategy. Additionally we propose masked differential privacy ({MaskDP}) to protect non-anonymized but privacy sensitive background information. MaskDP allows for controlling sensitive regions where differential privacy is applied, in contrast to applying DP on the entire input. This combined methodology provides strong privacy protection while minimizing the usual performance penalty of privacy preserving methods. Experiments on multiple challenging action recognition datasets demonstrate that our proposed techniques result in better utility-privacy trade-offs compared to standard differentially private training in the especially demanding $\epsilon<1$ regime.

==> algorithms/main_algorithm_old.tex <==
\begin{algorithm}
\caption{Data Anonymization for Assisted-DP}\label{alg:DataAnonymization}
\KwInput{Raw Video Dataset $ \mathcal{X} $\\}
$ m_{md}: \mathbb{R}^{H \times W \times 3} \rightarrow R_{\text{h}} $  \Comment{Person segmentation}
$ r_h: (\mathbb{R}^{H \times W \times F \times 3}, \mathbb{R}^{H \times W \times F}) \rightarrow \mathbb{R}^{H \times W \times F \times 3} $  \Comment{Video inpainting}
$ fa, fs: \mathbb{R}^{H \times W \times F \times 3} \rightarrow \mathbb{R}^{H \times W \times F \times 3} $  \Comment{$fa$, $fs$ denotes Avatars and Applying diffusion}

\KwResult{Anonymized Video Dataset $ \mathcal{X''} $}

\For{$ x $ in $ \mathcal{X} $}{
  $ R_{\text{h}} = m_{md}(x) $  \Comment{Identify person regions}
  $ x' = r_h(x, R_{\text{h}}) $  \Comment{Remove persons}
  $\mathcal{X^\prime}\leftarrow \mathcal{X^\prime} \cup \{x^\prime\}$
}

\For{$ x' $ in $ \mathcal{X'} $}{
  $ x'' = fs(fa(x')) $  \Comment{Generate avatar w/ pose, apply our {\color{blue}{temporal diffusion}} (see \Cref{sec:secv})}
  %Append $ x'' $ to $ \mathcal{X''} $
   $\mathcal{X^{\prime\prime}}\leftarrow \mathcal{X^{\prime\prime}} \cup \{x^{\prime\prime}\}$
}

\Return $\mathcal{X^{\prime\prime}}$
\end{algorithm}

\iffalse
\begin{algorithm}
\caption{Assisted-DP Training: Sample-based}\label{alg:ModelTraining}
\KwInput{Anonymized Video Dataset $ \mathcal{X''} $\\}
$ \mathcal{M}_\Theta:  \mathcal{T} \rightarrow \mathcal{Y} $ with weights $\Theta$ \Comment{Task classifier, where $\mathcal{T}$ and $\mathcal{Y}$ denote tokens and output classes, respectively. $y \in \mathcal{Y}$}
$ m_a: \mathbb{R}^{H \times W \times F \times 3} \rightarrow R_{\text{a}} $  \Comment{Avatar segmentation}
$ \text{Tokenize}: (\mathbb{R}^{H \times W \times F \times 3},R_{\text{a}}) \rightarrow (\mathcal{T}_{\text{B}}, \mathcal{T}_{\text{P}})$, where $\mathcal{T} = \mathcal{T}_{\text{B}} \cup \mathcal{T}_{\text{P}}$ \Comment{Decouple background and person tokens}
$ \mathcal{L}: \mathcal{Y} \rightarrow \mathbb{R}$, where  $\mathcal{L}$ is CE loss  \Comment{Loss functions}

\KwResult{AssistDP Trained model $\mathcal{M}_\Theta$}

\While{Training}{
  $x,y \sim \{\mathcal{X''}, \mathcal{Y}\}$ \Comment{Sample clip}
  $ R_{\text{a}} = m(x'') $  \Comment{Identify avatar regions}
  $ \mathcal{T}_{\text{B}}, \mathcal{T}_{\text{P}} = \text{Tokenize}(x'', R_{\text{a}}) $  \Comment{Separate tokens}
  $ L_{util} = \mathcal{L}(\mathcal{M}_\Theta(\mathcal{T}_{\text{P}}), y) $  
  $ L_{priv} = \mathcal{L}(\mathcal{M}_\Theta(\mathcal{T}_{\text{B}}), y) $ \\
  $ L_{total} = L_{util} + L_{priv} $  \Comment{Calculate losses}
  $ \nabla L_{util} = \frac{\partial L_{util}}{\partial W} $  
  $ \nabla L_{priv} = \text{DPSGD}(\frac{\partial L_{priv}}{\partial W}) $ \\
  $ \nabla L_{total} = \nabla L_{util} + \nabla L_{priv} $  \Comment{Backpropagation}
  $\Theta \gets \Theta - \eta \nabla L_{total} $
}
\Return $\mathcal{M}_\Theta$
\end{algorithm}
\fi

\begin{algorithm}
\caption{Assisted-DP Training: Batch-based}\label{alg:ModelTraining}
\KwInput{Anonymized Video Dataset $ \mathcal{X''} $\\}
$ \mathcal{M}_\Theta: \mathcal{T} \rightarrow \mathcal{Y} $ with weights $\Theta$ \Comment{Task classifier, where $\mathcal{T}$ and $\mathcal{Y}$ denote tokens and output classes, respectively. $y \in \mathcal{Y}$}
$ m_a: \mathbb{R}^{H \times W \times F \times 3} \rightarrow R_{\text{a}} $  \Comment{Avatar segmentation}
$ \text{Tokenize}: (\mathbb{R}^{H \times W \times F \times 3},R_{\text{a}}) \rightarrow (\mathcal{T}_{\text{B}}, \mathcal{T}_{\text{P}})$, where $\mathcal{T} = \mathcal{T}_{\text{B}} \cup \mathcal{T}_{\text{P}}$ \Comment{Decouple background and person tokens}
$ \mathcal{L}: \mathcal{Y} \rightarrow \mathbb{R}$, where  $\mathcal{L}$ is CE loss  \Comment{Loss functions}

\KwResult{AssistDP Trained model $\mathcal{M}_\Theta$}


\For{$t \in [T \cdot \frac{N}{K}]$}{
    Sample a batch ${K=(\mathcal{X}''_K, \mathcal{Y}_K})$ from  $\mathcal{X}'',\mathcal{Y}$  

    \For{$i \in \{1,2,\dots,|K|\}$}{
        $x'', y \gets K_i$\\
        $ R_{\text{a}} \gets m(x'') $  \Comment{Identify avatar regions}
        $ \mathcal{T}_{\text{B}}, \mathcal{T}_{\text{P}} \gets \text{Tokenize}(x'', R_{\text{a}}) $  \Comment{Separate tokens}

        $ L^i_{priv} \gets \mathcal{L}(\mathcal{M}_\Theta(\mathcal{T}_{\text{B}}), y) $ \\
        $\nabla L^i_{priv} \gets \frac{\partial L^i_{priv}}{\partial \Theta} \min(1, \frac{C}{\|\frac{\partial L^i_{priv}}{\partial \Theta}\|_2})$ \\

        $ L^i_{util} \gets \mathcal{L}(\mathcal{M}_\Theta(\mathcal{T}_{\text{P}}), y) $
    }

    $ \nabla L_{priv} \gets \frac{1}{|K|}\big(\sum_{i=1}^{|K|} \nabla L^i_{priv} + \mathcal{N}(0, \sigma^2\vec{I}) \big)  $ \\
    
    $ \nabla L_{util}  \gets \frac{\partial}{\partial\Theta}\frac{1}{|K|}\big(\sum_{i=1}^{|K|} L^i_{util}\big) $ 

    $ \nabla L_{total} \gets \nabla L_{util} + \nabla L_{priv} $ 

    $\Theta \gets \Theta - \eta \nabla L_{total} $
    % Update $ \Theta $ with $ \nabla L_{total} $
}

\Return $\mathcal{M}_\Theta$
\end{algorithm}


==> sec/0_abstract.tex <==
\begin{abstract}
The ABSTRACT is to be in fully justified italicized text, at the top of the left-hand column, below the author and affiliation information.
Use the word ``Abstract'' as the title, in 12-point Times, boldface type, centered relative to the column, initially capitalized.
The abstract is to be in 10-point, single-spaced type.
Leave two blank lines after the Abstract, then begin the main text.
Look at previous \confName abstracts to get a feel for style and length.
\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use options of \texttt{cvpr.sty} to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
For your results, however, you should not identify yourself and should not mention your participation in the challenge.
Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}


==> sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sections/3_background.tex <==
\section{Preliminaries}\label{sec:background}

%\subsection{Differential Privacy}
%
\newcommand{\Dataset}{\mathcal{D}}
%
Differential privacy (DP)~\cite{dwork2006calibrating} serves as a gold standard for ensuring the privacy of individuals' sensitive data.  
In simple terms, DP ensures that the output of an algorithm remains consistent regardless of whether a specific individual's data is included in the dataset. This means that an external observer who has access to the entire dataset except for one individual's information cannot determine with high probability whether that specific individual's data is part of the input. We provide a formal definition of DP below.
\begin{definition}[Differential Privacy~\cite{dwork2006calibrating}]\label{def:dp}
	Given $\epsilon > 0$ and $\delta > 0$, a randomized algorithm $\mathcal{A}$ satisfies $(\epsilon,\delta)$-differential privacy, if for all possible pairs of adjacent datasets $\Dataset$ and $\Dataset'$ differing by at most one record, denoted as $\Dataset\sim\Dataset'$, and for any possible set of outputs $S\subseteq Range(\mathcal{A})$, we have:
	\begin{equation*}
		\Pr[\mathcal{A}(\Dataset) \in S] \le e^\epsilon\Pr[\mathcal{A}(\Dataset') \in S] + \delta.
	\end{equation*}
\end{definition}
The parameter $\epsilon$ is referred to as the ``privacy budget'' or ``privacy cost,'' which balances the trade-off between privacy and utility. A smaller $\epsilon$ provides stronger privacy guarantees but might result in reduced utility. The parameter $\delta$ serves as a small failure probability, ensuring the robustness of the privacy mechanism. In the context of deep learning, DP techniques are employed during the model training process to protect the privacy of training data. The most popular algorithm, Differentially Private Stochastic Gradient Descent (DP-SGD)~\cite{abadi2016deep}, involves adding carefully calibrated noise to the clipped gradients computed during training, obscuring the contribution of individual data points.

==> sections/archive.tex <==
%Video anonymization technique hide the identity of individuals by replacing their bodies with synthesized virtual humans. However, this does not extend to the background, which could be informative for the target task but can still carry private information. To tackle this limitation, in this section, we present a hybrid approach that combines anonymized videos from the previous stage with differential privacy (DP).
%The idea is that, instead of training the model with DP-SGD, which can be overly pessimistic in terms of privacy, we apply DP exclusively when learning from the background regions of the video, which are not protected by our anonymization technique. This approach allows us to strike a better balance between utility and privacy compared to standard DP-SGD, as the DP noise doesn't significantly impact the human body regions, which are crucial for the activity recognition task.
%
%\subsubsection{Masked Differential Privacy}

\iffalse
\begin{figure}[!htb]
  \centering
  \includegraphics[width=0.7\textwidth]{imgs/rendering_pipeline.jpeg}
  \caption{Sample frames from a real video (i) and output video from our anonymization pipeline (iv). We also highlight the corresponding depth maps and synthesized virtual humans used to generate the final anonymized real video.}
  \label{fig:pipeline_demo}
\vspace{-3em}
\end{figure}

\subsection{Synthesizing Virtual Humans for Anonymization (Stage-I)} 
\label{sec:stage1}
We illustrate our end-to-end anonymization pipeline in \Cref{fig:data_generation} and list a more detailed description in \Cref{alg:DataAnonymization}.

Provided a 2D video recording $\RawVideoSample_i$, we leverage~\cite{goel2023humans} as our 3D pose estimation function $\PoseEstimation$ (Fig.~\ref{fig:data_generation}, \circled{\footnotesize 1}\ ) to acquire high-quality temporally consistent human motion information. While we find that this method may occasionally fail in scenarios with strong occlusions, it generally yields reliable results due to its usage of temporal information and is applicable to a wide range of data.

Rendering a synthetic human in place is not sufficient to completely hide a person in videos, since the generated avatar might not align with the original human contour in all cases. For this reason, we additionally apply an inpainting function $\VideoInpainting$~\cite{liCvpr22vInpainting} (Fig.~\ref{fig:data_generation}, \circled{\footnotesize 2}\ ), which removes the original person from the video before adding the virtual one, based on the mask $\RegionsPerson_i$  provided by a segmentation function $\PersonSegmentation$~\cite{li2022mask} which detects human presence regions in each frame.

For integrating a synthetic human into scenes, we developed our own data synthesizer $\Rendering$ 
 (Fig.~\ref{fig:data_generation}, \circled{\footnotesize 3}\ )  in contrast to using a commercial rendering engine, specifically for the capability to deploy our framework as an end-to-end solution in a headless computation setting. For human body parametrization, we leverage the SMPL-H body model~\cite{SMPL:2015, MANO:SIGGRAPHASIA:2017}, which offers flexibility, allowing adjustments in character attributes, such as height and body shape. Person diversity can easily be provided by textures as well as a variation of SMPL parameters. In our experiments, we apply 32 virtual humans of diverse ages and ethnicities, but much larger sets of characters can easily be integrated. 
 
 $\Rendering$ also provides us with depth maps and perfect pixel-wise masks $\RegionsAnonymized_i$, separating rendered anonymized humans from (potentially sensitive) background. $\RegionsAnonymized_i$ is different from the sanitization mask $\RegionsPerson_i$, since it describes pixel-wise synthetic data presence, while the $\RegionsPerson_i$ describes any pre-existing human presence, even if a valid pose and thereby a rendered human might not subsequently be generated. 
 
 Any eventual flaws in recognition of sensitive regions only affect task utility in this setup, since all non-synthesized regions will automatically be subject to subsequent masked differentially private training explained in~\Cref{sec:dp}.

Finally, a merging operation (Fig.~\ref{fig:data_generation}, \circled{\footnotesize 4}) combines the sanitized context information with the rendered human avatar, resulting in our anonymized data set.
\fi

\iffalse
In \Cref{sec:stage1}, we introduce our anonymization stage, 
which hides the identity of individuals by replacing their bodies with synthesized virtual ones.
Considering a dataset of raw video samples, each video contains regions that represent a human and are thereby considered to be highly sensitive while at the same time containing integral information for human action recognition. In order to avoid the application of low-$\epsilon$ noise for gradients affecting such image regions, we opt for replacing these regions completely with a synthetic avatar performing the same actions in place of the real human. 
\fi

\iffalse
\subsection{Human Action Recognition}
In this work, we focus on the task of human action recognition in videos, where the goal is to predict the correct action label for a given video sample. 
Formally, consider an activity recognition dataset $ \RawVideoDataset $ comprising $\DatasetSize$ samples $(\RawVideoSample_i, \LabelVector_i)\in\RawVideoDataset$, where $\RawVideoSample_i\in\mathbb{R}^{T\times H\times W\times C}$ is a video sample of length $T$ and spatial dimensions $H\times W$ with $C$ channels, and $\LabelVector_i\in\{0,1\}^{\NumClasses}$ is the corresponding one-hot encoded label vector denoting one of the $K$ activities. Our goal is to train a model $ \TaskModel $ to predict the correct label $\PredictedLabelVector$ for a given video sample $\RawVideoSample$. 
To this end, we seek to minimize a loss function $\LossFunction$, given by:
\begin{equation}
    \LossFunction(\TaskModel; \RawVideoDataset) = \sum_{i=1}^{\DatasetSize} \ell(\TaskModel(\RawVideoSample_i), \LabelVector_i),
\end{equation}
where $\TaskModel(\RawVideoSample_i)$ represents the predicted action label for video sample $\RawVideoSample_i$, $\LabelVector_i$ is the ground truth label, and $\ell$ is a suitable loss function, such as cross-entropy.

To preserve the privacy of the training data, we propose a hybrid approach that combines the use of synthetic data and differential privacy. Next, we briefly review the concept of differential privacy and its application in deep learning.
\fi

\iffalse
\paragraph{Training differential private neural networks.} In the context of deep learning, DP techniques are employed during the model training process to protect the privacy of training data. The most popular algorithm, Differentially Private Stochastic Gradient Descent (DP-SGD)~\cite{abadi2016deep}, involves adding carefully calibrated noise to the clipped gradients computed during training, obscuring the contribution of individual data points to the model updates. More specifically, for a randomly sampled mini-batch at each training iteration, DP-SGD computes per-sample gradients, clips them to a maximum norm, and then adds Gaussian noise to the average of the clipped gradients over the mini-batch. The resulting noisy gradients are then used to update the model parameters. The final privacy cost of DP-SGD (i.e., the value of $\epsilon$ for any given $\delta$) can then be computed based on the contributing factors, such as the noise scale, batch size, clipping norm, and the total number of training iterations, using a privacy accounting method, such as the moment accountant~\cite{abadi2016deep, wang2019subsampled} or the Fourier accountant~\cite{koskela2020computing, zhu2022optimal}.
\fi

\iffalse
\begin{figure*}[h!]
  \centering
\includegraphics[width=\textwidth]{imgs/synthesize_humans.pdf}

  \iffalse
  \includegraphics[width=0.99\textwidth]{imgs/pipeline.png}
  \fi
  \caption{Our Stage-I anonymization process is segmented into distinct steps for optimal performance and privacy preservation: \circled{\smaller 1} Pose estimation is conducted using a 4D human model, essential for subsequent avatar rendering. \circled{\smaller 2} The original human figures are then removed and inpainted using MaskDino and E2FGVI algorithms. \circled{\smaller 3} A synthetic avatar is rendered to replace the human subject. \circled{\smaller 4} The sanitized real-world video is merged with the generated avatar.}
  \label{fig:data_generation}
\end{figure*}
\fi




\iffalse
\begin{table}[htb!]
\centering
\caption{Performance evaluation in the context of differential privacy, with varying epsilon values and training methods.}
\begin{tabular}{llc|cccc}
\toprule
 \multicolumn{2}{c}{\multirow{2}{*}{Data}} & \multirow{2}{*}{Privacy} & \multicolumn{4}{c}{Acc/mPCA@$\epsilon$} \\
 \multicolumn{2}{c}{} &  & $1$ & $5$ & 10 & $\infty$ \\
\midrule
 \multirow{5}{*}{\centering\rotatebox{90}{\centering NTU RGB+D}} & Real World &  &  &  &  & \\
 & Synthetic &  &  &  &  &  \\
%\cmidrule{2-7}
 & Anonymized &  &  &  &  &  \\
 & Anonymized & \textsc{DP} &  &  &  &  \\
 & Anonymized & \textsc{MaskDP} & - & - & - & - \\
 \midrule[0.7pt]
 \multirow{5}{*}{\centering\rotatebox{90}{\centering TSH}} & Real World &  &  &  &  & \\
 & Synthetic &  &  &  &  &  \\
%\cmidrule{2-7}
 & Anonymized &  &  &  &  &  \\
 & Anonymized & \textsc{DP} &  &  &  &  \\
 & Anonymized & \textsc{MaskDP} & - & - & - & - \\
 \midrule[0.7pt]
 \multirow{5}{*}{\centering\rotatebox{90}{\centering HMDB-51}} & Real World &  &  &  &  & \\
 & Synthetic &  &  &  &  &  \\
%\cmidrule{2-7}
 & Anonymized &  &  &  &  &  \\
 & Anonymized & \textsc{DP} &  &  &  &  \\
 & Anonymized & \textsc{MaskDP} & - & - & - & - \\
\bottomrule
\end{tabular}
\caption{Comparative Analysis of Privacy Techniques on NTU-RGBD\cite{shahroudy2016ntu} contrasting the model's performance with synthetic and anonymized data under differential privacy (DP) and Masked Differential Privacy (MaskDP) across different epsilon values.}
\label{tab:dp_ntu}
\end{table}
\fi



\iffalse
\subsection{Evaluating Privacy by Replacement}
In order to evaluate how our synthetic person replacement strategy improves privacy, we perform retrieval experiments on paired synthetic and real world data. 
\noindent \textbf{Datasets and Preprocessing:} We utilize the \emph{NTU RGB+D} dataset for our privacy by replacement experiments. Each video clip spans 2 seconds, with 32 frames sampled per clip.

\noindent \textbf{Feature Extraction:} For each video in \(D\), \(D'\), and \(D''\), we sample 5 frames and employ a Vision Transformer (ViT) pretrained on ImageNet. The last layer of the ViT is discarded, and the resultant features serve as our primary descriptors.

\noindent \textbf{Retrieval-based Attacks:} Using the extracted features, we conduct k-NN retrieval attacks with k-values of 1, 3, 5, and 10. The similarity metric employed is cosine similarity on CLIP-Features. The primary objective is to ascertain the amount of information the synthetic datasets might leak about their real-world counterparts.

\noindent \textbf{Frechet Inception Distance (FID):} The FID between the generated data and the original data is computed to measure the similarity between the data distributions.

\noindent \textbf{Face Detection:} We deploy a modern face detection algorithm to discern if the original actors can be identified from the synthetic data samples.

\subsection{Evaluating Differentially Private Training}

\noindent \textbf{Datasets:} For these experiments, we focus on the \emph{NTU RGB+D} and \emph{Toyota Smarthome} datasets.

\noindent \textbf{Membership Attacks:} We assess the vulnerability of our model to membership inference attacks. The specifics of the attack methodology will be detailed in subsequent sections.

\noindent \textbf{Privacy Budget Ablation:} The model's performance is evaluated at varying privacy budgets, with \(\epsilon\) values of 1, 2, 4, and 8, and a fixed \(\delta\) of \(10^{-5}\). The results, presented in Table 1, showcase the trade-off between privacy and utility.

\noindent \textbf{Utility Experiments:} We juxtapose the performance of our model when trained solely on real-world data, purely on synthetic data, and a combination of both using our differential privacy mechanism. The results, illustrated in Figure 1, highlight the benefits of our mixed training approach.
\fi



\iffalse

\begin{table*}[htb!]
\centering
\caption{Performance evaluation in the context of differential privacy, with varying epsilon values and training methods.}
\begin{tabular}{c|l|c|ccccc}
\toprule
 & Data & Privacy & $\epsilon=1$ & $\epsilon=2$ & $\epsilon=4$ & $\epsilon=8$ & $\epsilon=\infty$ \\
\midrule
\multirow{5}{*}{\centering\rotatebox{90}{\centering MViTv2S~\cite{li2021improved}}} 
& Real World &  & - & - & - & - & - \\
& Synthetic &  & - & - & - & - & - \\
\cmidrule{2-8}
& Anonymized &  & - & - & - & - & - \\
& Anonymized &  & - & - & - & - & - \\
& Anonymized & MaskDP & - & - & - & - & - \\
\bottomrule
\end{tabular}
\caption{Comparative Analysis of Privacy Techniques on NTU-RGBD\cite{shahroudy2016ntu} contrasting the model's performance with synthetic and anonymized data under differential privacy (DP) and Masked Differential Privacy (MaskDP) across different epsilon values.}
\label{tab:dp_ntu}
\end{table*}

\begin{table*}[htb!]
\centering
\caption{Performance evaluation in the context of differential privacy, with varying epsilon values and training methods.}
\begin{tabular}{c|l|c|ccccc}
\toprule
 & Data & Privacy & $\epsilon=1$ & $\epsilon=2$ & $\epsilon=4$ & $\epsilon=8$ & $\epsilon=\infty$ \\
\midrule
\multirow{5}{*}{\centering\rotatebox{90}{\centering MViTv2S~\cite{li2021improved}}} 
& Real World &  & - & - & - & - & - \\
& Synthetic &  & - & - & - & - & - \\
\cmidrule{2-8}
& Anonymized &  & - & - & - & - & - \\
& Anonymized &  & - & - & - & - & - \\
& Anonymized & MaskDP & - & - & - & - & - \\
\bottomrule
\end{tabular}
\caption{Comparative Analysis of Privacy Techniques on Toyota Smarthome\cite{das2019toyota} contrasting the model's performance with synthetic and anonymized data under differential privacy (DP) and Masked Differential Privacy (MaskDP) across different epsilon values.}
\label{tab:dp_tsh}
\end{table*}

\begin{table*}[htb!]
\centering
\caption{Performance evaluation in the context of differential privacy, with varying epsilon values and training methods.}
\begin{tabular}{c|l|c|ccccc}
\toprule
 & Training Data & Privacy & $\epsilon=1$ & $\epsilon=2$ & $\epsilon=4$ & $\epsilon=8$ & $\epsilon=\infty$ \\
\midrule
\multirow{5}{*}{\centering\rotatebox{90}{\centering MViTv2S~\cite{li2021improved}}} 
& Real World &  & - & - & - & - & - \\
& Synthetic &  & - & - & - & - & - \\
\cmidrule{2-8}
& Anonymized &  & - & - & - & - & - \\
& Anonymized &  & - & - & - & - & - \\
& Anonymized & MaskDP & - & - & - & - & - \\
\bottomrule
\end{tabular}
\caption{Comparative Analysis of Privacy Techniques on Toyota Smarthome\cite{das2019toyota} contrasting the model's performance with synthetic and anonymized data under differential privacy (DP) and Masked Differential Privacy (MaskDP) across different epsilon values.}
\label{tab:dp_hmdb51}
\end{table*}

\fi

==> tables/dp.tex <==
\iffalse
\begin{table}[htb!]
\centering
\caption{Performance evaluation in the context of differential privacy, with varying epsilon values and training methods.}
\begin{tabular}{l|c|cccc}
\toprule
 \multirow{2}{*}{Data} & \multirow{2}{*}{Privacy} & \multicolumn{4}{c}{Acc@$\epsilon$} \\
  &  & $1$ & $5$ & $10$ & $\infty$ \\
\midrule
 Real World$\dagger$ &  & &  &  & 71.2 \\
 Real World &  & &  &  & $33^{*}$ \\
 Real World & \textsc{DP} & &  &  & \\
 Synthetic &  &  &  &  &  \\
\cmidrule{1-6}
 Anonymized &  &  &  &  & $21^{*}$ \\
 Anonymized & \textsc{DP} & $12.9^{*}$ & $17.9^{*}$  & $17.3^{*}$ &  \\
 Anonymized & MaskDP & $18.1^{*}$ & $18.3^{*}$ & $19.2^{*}$ &   \\
\bottomrule
\end{tabular}
\caption{Comparative Analysis of Privacy Techniques on Toyota Smarthome\cite{das2019toyota} contrasting the model's performance with synthetic and anonymized data under differential privacy (DP) and Masked Differential Privacy (MaskDP) across different epsilon values.}
\label{tab:dp_tsh}
\end{table}

\begin{table}[htb!]
\centering
\caption{Performance evaluation in the context of differential privacy, with varying epsilon values and training methods.}
\begin{tabular}{l|c|cccc}
\toprule
 \multirow{2}{*}{Data} & \multirow{2}{*}{Privacy} & \multicolumn{4}{c}{Acc@$\epsilon$} \\
  &  & $1$ & $5$ & $10$ & $\infty$ \\
\midrule
 Real World &  & &  &  &  \\
 Real World & \textsc{DP} & &  &  & \\
 Synthetic &  &  &  &  &  \\
\cmidrule{1-6}
 Anonymized &  &  &  &  &  \\
 Anonymized & \textsc{DP} &  &   &  &  \\
 Anonymized & MaskDP & - & - & - & - \\
\bottomrule
\end{tabular}
\caption{Comparative Analysis of Privacy Techniques on HMDB-51\cite{das2019toyota} contrasting the model's performance with synthetic and anonymized data under differential privacy (DP) and Masked Differential Privacy (MaskDP) across different epsilon values.}
\label{tab:dp_hmdb51}
\end{table}
\fi

\iffalse
\begin{table}[htb!]
\centering
\begin{tabular}{l|c|cccc}
\toprule
 \multirow{2}{*}{Data} & \multirow{2}{*}{Privacy} & \multicolumn{4}{c}{Recall@$K$} \\
  &  & $1$ & $5$ & $10$ & $50$ \\
\midrule
 Real World &  & &  &  &  \\
 Real World & \textsc{DP} & &  &  & \\
 Anonymized & \textsc{DP} &  &   &  &  \\
 Anonymized & MaskDP & - & - & - & - \\
\bottomrule
\end{tabular}
\caption{Privacy a }
\label{tab:privacy_recall}
\end{table}
\fi

\iffalse
% HMDB
  \multirow{6}{*}{\rotatebox[origin=c]{90}{\centering HMDB-51}}
 & Real~\cite{luo2024differentially}  & \textsc{DP} & \multicolumn{4}{c}{------}                                                             & $51.7$~\ch{} & $56.5$~\ch{} & ---~\ch{}  \\
 & Real       & \textsc{DP} & $2.3$~\ch{}    & $3.9$~\ch{}     & $6.6$~\ch{}      & $36.7$~\ch{}      & $65.8$~\ch{}      & $73.3$~\ch{}      & $76.1$~\ch{}     \\
 & Render     & \textsc{DP} & $2.4$~\ch{0.1} & $3.3$~\ch{-0.6} & $4.5$~\ch{-2.1}  & $13.5$~\ch{-23.2} & $45.7$~\ch{-20.1} & $57.7$~\ch{-16}   & $60.9$~\ch{-15.2}  \\
 & Render     & MaskDP      & $8.2$~\ch{5.9} & $7.8$~\ch{3.9}  & $26.2$~\ch{19.6} & $39.7$~\ch{3.0}   & $51.5$~\ch{-14.3} & $50.9$~\ch{-22.4} & $60.9$~\ch{-15.2} \\
 & Rend.+Diff & \textsc{DP} & ---~\ch{}      & $64.3$~\ch{}       & ---~\ch{}        & ---~\ch{}         & 65.8\ch{}         & ---~\ch{}         & ---~\ch{}  \\
 & Rend.+Diff & MaskDP      & ---~\ch{}      & ---~\ch{}       & ---~\ch{}        & ---~\ch{}         & ---~\ch{}         & ---~\ch{}         & ---~\ch{} \\

% ucf
   \cmidrule{1-10}
  \multirow{6}{*}{\rotatebox[origin=c]{90}{\centering UCF-101}}
 & Real~\cite{luo2024differentially} & \textsc{DP} & \multicolumn{4}{c}{------} & $75.1$~\ch{} & $78.2$~\ch{} & ---~\ch{}    \\
 & Real       & \textsc{DP} & $1.2$~\ch{}     & $2.0$~\ch{}      & $66.7$~\ch{}      & $85.5$~\ch{}      & $93.1$~\ch{}      & $95.3$~\ch{}      & $97.2$~\ch{}    \\
 & Render     & \textsc{DP} & $0.7$~\ch{-0.5} & $1.5$~\ch{-0.5}  & $19.5$~\ch{-47.2} & $65.6$~\ch{-19.9} & $77.1$~\ch{-18.2} & $82.1$~\ch{-15.1} & $85.9$~\ch{-11.3}      \\
 & Render     & MaskDP      & $5.0$~\ch{3.8}  & $15.4$~\ch{13.4} & $36.6$~\ch{-30.1} & $63.9$~\ch{-21.6} & $74.5$~\ch{-20.6} & $73.9$~\ch{-23.3} & $85.9$~\ch{-11.3}     \\
 & Rend.+Diff & \textsc{DP} & ---~\ch{}       & ---~\ch{}        & ---~\ch{}         & ---~\ch{}         & ---~\ch{}         & ---~\ch{}         & ---~\ch{}  \\
 & Rend.+Diff & MaskDP      & ---~\ch{}       & ---~\ch{}        & ---~\ch{}         & ---~\ch{}         & ---~\ch{}         & ---~\ch{}         & ---~\ch{} \\

\fi

==> tables/retrieval.tex <==
\begin{table}[htb!]
\centering
\caption{Analysis of background retrieval performance given varying training data and training schemes.}
\begin{tabular}{c|l|c|c|cc} 
\toprule
 & Training Data & Privacy & $\epsilon$ & R@1 & R@5 \\
\midrule
\multirow{9}{*}{\centering\rotatebox{90}{\centering MViTv2S~\cite{li2021improved}}} 
& Real World & None & & - & - \\
& Anonymized & Person & & - & - \\
\cmidrule{2-6} 
& Anonymized & DP & 1 & - & - \\
& Anonymized & DP & 4 & - & - \\
& Anonymized & DP & 8 & - & - \\
& Anonymized & MaskDP & 1 & - & - \\
& Anonymized & MaskDP & 4 & - & - \\
& Anonymized & MaskDP & 8 & - & - \\
\bottomrule
\end{tabular}
\end{table}

